Chandra Resolves the T Tauri Binary System RW Aur

RW Aur is a multiple T Tauri system consisting of an early-K type primary (A) and a K5 companion (B) at a separation of 1.4 arcsec. RW Aur A drives a bipolar optical jet that is well-characterized optically. We present results of a sensitive Chandra observation whose primary objective was to search for evidence of soft extended X-ray emission along the jet, as has been seen for a few other nearby T Tauri stars. The binary is clearly resolved by Chandra and both stars are detected as X-ray sources. The X-ray spectra of both stars reveal evidence for cool and hot plasma. Suprisingly, the X-ray luminosity of the less-massive secondary is at least twice that of the primary and is variable. The disparity is attributed to the primary whose X-ray luminosity is at the low end of the range for classical T Tauri stars of similar mass based on established correlations. Deconvolved soft-band images show evidence for slight outward elongation of the source structure of RW Aur A along the blueshifted jet axis inside the central arcsecond. In addition, a faint X-ray emission peak is present on the redshifted axis at an offset of 1.2 +- 0.2 arcsec from the star. Deprojected jet speeds determined from previous optical studies are too low to explain this faint emission peak as shock-heated jet plasma. Thus, unless flow speeds in the redshifted jet have been underestimated, other mechanisms such as magnetic jet heating may be involved.

==> table1.tex <==
%% TABLE 1                                                                                                                                                                                              
\begin{deluxetable}{lccccccccc}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{Properties of RW Aur}
\tablehead{
           \colhead{Object}             &
           \colhead{Type}               &
           \colhead{log Age}                &
           \colhead{M$_{*}$}            &
           \colhead{R$_{*}$}            &
           \colhead{T$_{eff}$}          &
           \colhead{log L$_{*}$}            &
           \colhead{A$_{v}$}            &
           \colhead{d}                  &
           \colhead{Refs.}             \\
           \colhead{}                   &
           \colhead{}                   &
           \colhead{(y)}                   &
           \colhead{(M$_{\odot}$)}         &
           \colhead{(R$_{\odot}$)}         &
           \colhead{(K)}                   &
           \colhead{(L$_{\odot}$)}                   &
           \colhead{(mag)}                   &
           \colhead{(pc)}                &
           \colhead{}
}
\startdata
RW Aur A &  K3         & ...            &  0.9            & 1.1    & ...        & $-$0.30             & 0.55             & 140 & 1    \\
RW Aur A &  K1$\pm$2   & 6.92$\pm$0.31  &  1.34$\pm$0.18  & ...   & 5082       & 0.23$\pm$0.14       & 0.39$\pm$0.33    & 140 & 2   \\
RW Aur B &  K5         & 7.13$\pm$0.18  &  0.93$\pm$0.09  & ...   & 4395       & $-$0.40$\pm$0.10    & 1.56$\pm$0.24    & 140 & 2   \\
\enddata
\tablecomments{A$_{v}$ = 1.11 A$_{\rm V}$. \\
1. Ingleby et al. (2013).  \\
2. White \& Ghez (2001).
}
\end{deluxetable}



==> table2.tex <==
%% TABLE 2                                                                                                                                                                 
\begin{deluxetable}{lllcccccl}
\tabletypesize{\scriptsize}
\tablewidth{0pt}
\tablecaption{ X-ray Properties of RW Aur (Chandra ACIS-S)}
\tablehead{
         \colhead{Name} &
           \colhead{R.A.}               &
           \colhead{decl.}              &
           \colhead{Net Counts}         &
           \colhead{H.R.}               &
           \colhead{E$_{50}$}           &
           \colhead{P$_{const}$}             &
           \colhead{log L$_{x}$}             &
           \colhead{2MASS Identification(offset)}      \\
           \colhead{}   &
           \colhead{(J2000)}                 &
           \colhead{(J2000)} &
           \colhead{(cts)}                                          &
           \colhead{}                                          &
           \colhead{(keV)}                                          &
           \colhead{}                                          &
           \colhead{(ergs s$^{-1}$)}                                          &
           \colhead{(arcsec)}
                                  }
\startdata
RW Aur A         & 05 07 49.54 & $+$30 24 04.95 & 986 $\pm$ 33  & $-$0.72 & 1.00 & 0.96     & 29.44 & J050749.538$+$302405.07 (0.12) \\
RW Aur B         & 05 07 49.43 & $+$30 24 04.55 & 2909 $\pm$ 33 & $-$0.73 & 1.12 & $<$0.001 & 29.89 & ... \\ 
\enddata
\tablecomments{
The nominal pointing position for
the observation was (J2000.0) RA = 05$^h$ 07$^m$ 50.33$^s$,
decl. = $+$30$^{\circ}$ 23$'$ 59$''$.7.
X-ray data are from CCD7 (ACIS chip S3) using events in the 0.2 - 8 keV range inside a
circular source extraction region of radius 0$''$.9 centered on the X-ray peak.
Events common to both sources (33 events) where the two circles overlap are excluded.
Tabulated quantities are: J2000.0 X-ray position (R.A., decl.), total source counts accumulated
in a 54,482 s exposure,  hardness ratio H.R. = (H$-$S)/(H$+$S) where H = counts(2-8 keV)
and S = counts(0.2 - 2 keV), median photon  energy (E$_{50}$),
probability of constant count-rate determined by the Gregory-Loredo
algorithm (P$_{const}$); unabsorbed X-ray luminosity (0.3 - 8 keV at d = 140 pc; L$_{x}$ is model-dependent, see  Table 3),
and 2MASS near-IR  counterpart identification.
The offset (in parenthesis) is given in arc seconds between the X-ray and 2MASS counterpart position.
The X-ray offset of B from A is 1.$''$48 along P.A. = 254.3$^{\circ}$.}


\end{deluxetable}


==> table3.tex <==
% TABLE3.TEX                                                                                                                                
\begin{deluxetable}{lllll}
\tabletypesize{\scriptsize}
%\tablewidth{33pc}                                                                                                                           
\tablewidth{0pc}
\tablecaption{{\em Chandra} Spectral Fits of RW Aur A and B
   \label{tbl-1}}
\tablehead{
\colhead{Parameter}      &
\colhead{ }              &
\colhead{  }
}
\startdata
Object                                  & RW Aur A                 & RW Aur A                  & RW Aur B                  & RW Aur B     \nl
Model\tablenotemark{a}                  & 2T\tablenotemark{a}      & 1T $+$ PL\tablenotemark{b}& 2T\tablenotemark{a}       & 2T\tablenotemark{a}  \nl
N$_{\rm H}$ (10$^{20}$ cm$^{-2}$)       & \{6.5\}\tablenotemark{c} & \{6.5\}\tablenotemark{c}  & 4.3 [2.3 - 6.5]           & \{22.4\}\tablenotemark{d} \nl
kT$_{1}$ (keV)                          & 0.65 [0.58 - 0.75]       & 0.73 [0.64 - 0.79]        & 0.98 [0.82 - 1.01]        & 0.39 [0.35 - 0.42] \nl
kT$_{2}$ (keV)                          & \{20.\}\tablenotemark{e} & ...                       & 3.15 [2.58 - 4.06]        & 2.39 [2.09 - 2.74] \nl
$\Gamma_{ph}$                           & ...                      & $-$0.04 [$-$0.76 - 0.59]  & ...                       & ... \nl
norm$_{1}$ (10$^{-5}$)\tablenotemark{f} & 3.30 [2.46 - 4.15]       & 5.03 [4.14 - 5.84]        & 6.80 [4.35 - 9.85]        & 14.0 [11.4 - 16.8] \nl
norm$_{2}$  (10$^{-5}$)\tablenotemark{f}& 2.86 [2.29 - 3.42]       & 0.10 [0.03 - 0.26]        & 13.3 [11.1 - 15.3]        & 18.4 [16.8 - 19.9] \nl
Ne                                      & 1.53 [0.72 - 2.6]        & 0.76 [0.00 - 1.59]        & 1.69 [0.09 - 3.30]        & 2.16 [1.73 - 2.69] \nl
Fe                                      & 0.39 [0.29 - 0.57]       & 0.27 [0.21 - 0.35]        & 0.36 [0.24 - 0.50]        & 0.22 [0.14 - 0.33] \nl
$\chi^2$/dof                            & 83.3/64                  & 68.9/63                   & 116.1/124                 & 137.4/125          \nl 
$\chi^2_{red}$                          & 1.30                     & 1.09                      & 0.94                      & 1.10 \nl
F$_{\rm X}$ (10$^{-13}$ ergs cm$^{-2}$ s$^{-1}$)   & 0.97 (1.17)   & 1.19 (1.39)               & 2.93 (3.31)\tablenotemark{g} & 2.75 (5.16)  \nl
F$_{\rm X,1}$ (10$^{-13}$ ergs cm$^{-2}$ s$^{-1}$) & 0.51 (0.67)   & 0.64 (0.83)               & 1.08 (1.27)               & 0.96 (2.55) \nl
F$_{\rm X,2}$ (10$^{-13}$ ergs cm$^{-2}$ s$^{-1}$) & 0.46 (0.50)   & 0.55 (0.56)               & 1.85 (2.04)               & 1.79 (2.61) \nl
log L$_{\rm X}$ (ergs s$^{-1}$)                    & 29.44         & 29.51                     & 29.89                     & 30.08   \nl
log [L$_{\rm X}$/L$_{*}$]                          & $-$3.84       & $-$3.77                   & $-$3.29                   & $-$3.10 \nl
\enddata
\tablecomments{
Based on  XSPEC (vers. 12.7.1) fits of the background-subtracted ACIS-S spectra binned
to a minimum of 10 counts per bin using 54,482 sec of  exposure time. The spectra were
modeled with an absorbed  two-temperature (2T) $vapec$ optically thin plasma 
model or an absorbed one-temperature (1T) $vapec$ plasma $+$ a power-law (PL) component. 
The Ne and Fe abundances were allowed to vary during the fit but their abundances in the cool and hot 
thermal plasma components were constrained  to be equal.
The tabulated parameters
are absorption column density (N$_{\rm H}$), plasma energy (kT),
photon power-law index ($\Gamma_{ph}$),
XSPEC component normalization (norm), neon (Ne) and iron (Fe) abundances. 
Abundances are referenced to  
the solar values of Anders \& Grevesse (1989).
Square brackets enclose 90\% confidence intervals. 
Quantities enclosed in curly braces were held fixed during fitting.
The total X-ray flux (F$_{\rm X}$) and fluxes associated with each model component
(F$_{\rm X,i}$)  are the absorbed values in the 0.3 - 8 keV range, followed in
parentheses by  unabsorbed values.
The total X-ray luminosity L$_{\rm X}$  is the  unabsorbed
value in the 0.3 - 8 keV range and  assumes a
distance of 140 pc. The adopted stellar luminosities are  L$_{*}$ = 0.5 L$_{\odot}$ for
RW Aur A (Ingleby et al. 2013) and L$_{*}$ = 0.4  L$_{\odot}$ for RW Aur B (White \& Ghez 2001).}
\tablenotetext{a}{XSPEC model of form $wabs$$\cdot$($vapec$ $+$ $vapec$) .}
\tablenotetext{b}{XSPEC model of form $wabs$$\cdot$($vapec$ $+$ $pow$) .}
\tablenotetext{c}{Held fixed during fitting at upper 90\% confidence bound.}
\tablenotetext{d}{Held fixed during fitting at the value inferred from A$_{\rm V}$ = 1.4 mag
                  (White \& Ghez (2001) and the A$_{\rm V}$ to N$_{\rm H}$ conversion of Vuong et al. (2003).}
\tablenotetext{e}{Fits require high but poorly-constrained hot-component temperature.
                  Value held fixed during fitting at lower 90\% confidence bound.}
\tablenotetext{f}{For thermal $vapec$ models, the norm is related to the volume emission measure
                  (EM = n$_{e}^{2}$V)  by
                  EM = 4$\pi$10$^{14}$d$_{cm}^2$$\times$norm, where d$_{cm}$ is the stellar
                  distance in cm. At d = 140 pc this becomes
                  EM = 2.35$\times$10$^{56}$ $\times$ norm (cm$^{-3}$). }  
\tablenotetext{g}{The flux is variable. The 0.3 - 8 keV fluxes during the first and second halves
                  of the observation in units of 10$^{-13}$ ergs cm$^{-2}$ s$^{-1}$
                  were F$_{\rm X}$  = 2.33 (2.65) and F$_{\rm X}$ = 3.48 (3.90)  
                  where the value in parentheses is unabsorbed. The corresponding 
                  X-ray luminosities are log L$_{x}$ = 29.79 and 29.96 (ergs s$^{-1}$).}
\end{deluxetable}

